LASHED: LLMs And Static Hardware Analysis for Early Detection of RTL Bugs

While static analysis is useful in detecting early-stage hardware security bugs, its efficacy is limited because it requires information to form checks and is often unable to explain the security impact of a detected vulnerability. Large Language Models can be useful in filling these gaps by identifying relevant assets, removing false violations flagged by static analysis tools, and explaining the reported violations. LASHED combines the two approaches (LLMs and Static Analysis) to overcome each other's limitations for hardware security bug detection. We investigate our approach on four open-source SoCs for five Common Weakness Enumerations (CWEs) and present strategies for improvement with better prompt engineering. We find that 87.5% of instances flagged by our recommended scheme are plausible CWEs. In-context learning and asking the model to 'think again' improves LASHED's precision.

==> Sections/preamble/preamble-old.tex <==
% \usepackage[noadjust]{cite}
% \usepackage{pslatex} % -- times instead of computer modern, especially for the plain article class
% \usepackage[colorlinks=false,bookmarks=false]{hyperref}
\usepackage[utf8]{inputenc}
% \usepackage[dvipsnames,table]{xcolor}
\usepackage[most]{tcolorbox}

\usepackage{booktabs}

\usepackage{graphicx}
\usepackage{multirow}
%\usepackage{cite}
% \usepackage[noadjust]{cite} 
\usepackage{setspace}
%
\usepackage{amsmath}
%\usepackage{amssymb} %decomment for arXiv
\usepackage{amsfonts} %
\usepackage{calligra} %
\usepackage{mathtools}
\usepackage{amsthm} % for neater definitions
\usepackage[hidelinks,bookmarks=false]{hyperref}
% \usepackage{dblfloatfix} %allows floats to be at bottom of page
% \usepackage{array}
\usepackage{enumitem}

% \usepackage{caption}
% \usepackage{subcaption}

\usepackage{pgfplots}
\usepackage{pgfplotstable}
\usepgfplotslibrary{statistics}

% \usepackage{subcaption}
% \captionsetup{compatibility=false}

%tikz and associated stuff
%\usepackage{tikz}
% \usepackage{verbatim}
%\usetikzlibrary{shapes,backgrounds}
%\usetikzlibrary{arrows,fit,automata,positioning,decorations,calc}
%\usetikzlibrary{spy}
%\usetikzlibrary{matrix,chains,decorations.pathreplacing}
%\usetikzlibrary{arrows.meta}

% \usepackage{caption}
% \usepackage{subcaption} 

%%%% fix to use subcaptions in IEEE template ######
\makeatletter
\let\MYcaption\@makecaption
\makeatother
\usepackage[font=footnotesize]{subcaption}
\makeatletter
\let\@makecaption\MYcaption
\makeatother
%%%%% end fix
\renewcommand\thesubfigure{(\alph{subfigure})}
\captionsetup[subfigure]{labelformat=simple}

\usepackage{comment}
\usepackage{listings}

\usepackage{circledsteps}

\usetikzlibrary{patterns}

% \usepackage[percent]{overpic}

% \usepackage[english]{babel}
\usepackage{blindtext}

\usepackage{acronym}
%\usepackage[subtle]{savetrees}

\usepackage{xcolor, colortbl}

%\usepackage{flushend} % even out the last page, but use only at the end when there is a bibliography

\newcommand\defeq{\stackrel{\mathclap{\scriptsize\mbox{def}}}{=}}
\newcommand{\code}[1]{{\small{\texttt{#1}}}}

% fatter TT font
\renewcommand*\ttdefault{txtt}
% another TT, suggested by Alex
% \usepackage{inconsolata}
% \usepackage[T1]{fontenc} % needed as well?

\usepackage{float}
\usepackage{textcomp}

\newcommand{\todo}[1]{{\color{red}\textsc{\hl{[TODO:]}} #1}}
\newcommand{\hammond}[1]{{\color{blue} Hammond: #1}}
\newcommand{\matthew}[1]{{\color{red} Matthew: #1}}
\newcommand{\changed}[1]{{\color{red}#1}}

%\theoremstyle{definition}
%\newtheorem{definition}{Definition}[section] % definition numbers are dependent on theorem numbers
%\theoremstyle{example}
%\newtheorem{example}[definition]{Example} % same for example numbers
%\theoremstyle{theorem}
%\newtheorem{theorem}[definition]{Theorem}
%\newtheorem{lemma}[definition]{Lemma}
%\newtheorem{defn}{definition}[section]
%\newtheorem{exmp}{example}[section]
%\newtheorem{remark}[definition]{Remark}

\usepackage{algorithm}
\usepackage{algorithmic}

\usepackage{url}

% Ben extra packages ========================================
\usepackage[all=normal,paragraphs=tight, floats=tight,indent=tight]{savetrees}
\usepackage{pifont}
\usepackage{framed}
\usepackage{soul}
% \usepackage{booktabs}  
\usepackage{csquotes}
\usepackage{multirow}
\usepackage{array}
\newcolumntype{L}[1]{>{\raggedright\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{C}[1]{>{\centering\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{R}[1]{>{\raggedleft\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{H}{>{\collectcell\lstinline}l<{\endcollectcell}}
\usepackage{url}
\MakeOuterQuote{"}
% \usepackage[caption=false,font=normalsize,labelfont=sf,textfont=sf]{subfig} % for compsoc
\usepackage[caption=false,font=footnotesize,labelformat=simple]{subfig} % caption=false is needed for IEEE template
% \renewcommand\thesubfigure{(\alph{subfigure})} % labelformat simple removes the parentheses, this adds them back so \autoref(subfigure label) gives you Fig. X(a), etc.
% \captionsetup[subfigure]{labelformat=simple}

\newcommand{\todoblock}[1]{\noindent\definecolor{shadecolor}{RGB}{252, 217, 217}\colorbox{shadecolor}{\parbox{\columnwidth}{{#1}}}}
\newcommand{\todoblockblue}[1]{\noindent\definecolor{shadecolor}{RGB}{214, 254, 255}\colorbox{shadecolor}{\parbox{\columnwidth}{{#1}}}}
\newcommand{\todoblockgreen}[1]{\noindent\definecolor{shadecolor}{RGB}{175, 255, 191}\colorbox{shadecolor}{\parbox{\columnwidth}{{#1}}}}
\newcommand{\findcite}[1]{\sethlcolor{yellow}\hl{[#1]}}
% \usepackage[bookmarks=false]{hyperref}
\def\sectionautorefname{Section}
\def\subsectionautorefname{Section}
\def\subsubsectionautorefname{Section}
\def\algorithmautorefname{Algorithm}
\def\figureautorefname{Figure}
\def\subfigureautorefname{Figure}
\def\tableautorefname{Table}
%\renewcommand\thesubfigure{(\alph{subfigure})} % to get the (a) when using autoref with a subfig
% \renewcommand{\figurename}{Fig.}
\newcommand{\hlr}[1]{{\color{red}{\hl{#1}}}}
% \newcommand{\bt}[1]{#1}
\newcommand{\bt}[1]{{\color{blue}{#1}}}
\newcommand{\rt}[1]{{\color{red}{#1}}}
\newcommand{\pt}[1]{{\color{purple}{#1}}}
\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%
% \newcommand{\ts}[1]{\textsuperscript{#1}}
% \newcommand{\snip}{\vspace{-1.5em}}
\newcommand{\snip}{}
\newcommand{\sol}{LASHED}

\pgfplotsset{compat=1.18}
% ======================================== 


==> Sections/preamble/preamblelistingsconf.tex <==
\definecolor{mygreen}{rgb}{0,0.6,0}
\definecolor{mygray}{rgb}{0.5,0.5,0.5}
\definecolor{mymauve}{rgb}{0.58,0,0.82}

\makeatletter
\let\old@lstKV@SwitchCases\lstKV@SwitchCases
\def\lstKV@SwitchCases#1#2#3{}
\makeatother
\usepackage{lstlinebgrd}
\makeatletter
\let\lstKV@SwitchCases\old@lstKV@SwitchCases

\lst@Key{numbers}{none}{%
    \def\lst@PlaceNumber{\lst@linebgrd}%
    \lstKV@SwitchCases{#1}%
    {none:\\%
     left:\def\lst@PlaceNumber{\llap{\normalfont
                \lst@numberstyle{\thelstnumber}\kern\lst@numbersep}\lst@linebgrd}\\%
     right:\def\lst@PlaceNumber{\rlap{\normalfont
                \kern\linewidth \kern\lst@numbersep
                \lst@numberstyle{\thelstnumber}}\lst@linebgrd}%
    }{\PackageError{Listings}{Numbers #1 unknown}\@ehc}}
\makeatother

\usepackage{lstlinebgrd} % see http://www.ctan.org/pkg/lstaddons

\lstset{ 
  escapeinside={(*@}{@*)},
%   backgroundcolor=\color{white},   % choose the background color; you must add \usepackage{color} or \usepackage{xcolor}; should come as last argument
  basicstyle=\scriptsize,        % the size of the fonts that are used for the code
  upquote=true,
%   breakatwhitespace=false,         % sets if automatic breaks should only happen at whitespace
  breaklines=true,                 % sets automatic line breaking
%   captionpos=b,                    % sets the caption-position to bottom
  commentstyle=\color{mygreen},    % comment style
%   deletekeywords={...},            % if you want to delete keywords from the given language
%   escapeinside={\%*}{*)},          % if you want to add LaTeX within your code
%   extendedchars=true,              % lets you use non-ASCII characters; for 8-bits encodings only, does not work with UTF-8
  frame=single,	                   % adds a frame around the code
%   keepspaces=true,                 % keeps spaces in text, useful for keeping indentation of code (possibly needs columns=flexible)
  keywordstyle=\color{blue},       % keyword style
  language=C,                 % the language of the code
%   morekeywords={*,...},            % if you want to add more keywords to the set
  numbers=left,                    % where to put the line-numbers; possible values are (none, left, right)
  numbersep=5pt,                   % how far the line-numbers are from the code
  numberstyle=\tiny\color{mygray}, % the style that is used for the line-numbers
%   rulecolor=\color{black},         % if not set, the frame-color may be changed on line-breaks within not-black text (e.g. comments (green here))
%   showspaces=false,                % show spaces everywhere adding particular underscores; it overrides 'showstringspaces'
  showstringspaces=false,          % underline spaces within strings only
%   showtabs=false,                  % show tabs within strings adding particular underscores
%   stepnumber=1,                    % the step between two line-numbers. If it's 1, each line will be numbered
  stringstyle=\color{mymauve},     % string literal style
%   tabsize=2,	                   % sets default tabsize to 2 spaces
%   title=\lstname                   % show the filename of files included with \lstinputlisting; also try caption instead of title
%   %framesep=0pt,framerule=0pt,
%   %aboveskip=0pt,belowskip=0pt
}


% Define JSON language style

\definecolor{delim}{RGB}{20,105,176}
\definecolor{numb}{RGB}{106, 109, 32}
\definecolor{string}{rgb}{0.64,0.08,0.08}

\lstdefinelanguage{json}{
    % showspaces=false,
    showtabs=false,
    breaklines=true,
    % postbreak=\raisebox{0ex}[0ex][0ex]{\ensuremath{\color{gray}\hookrightarrow\space}},
    breakatwhitespace=true,
    basicstyle=\scriptsize,
    showstringspaces=false,
    upquote=true,
    morestring=[b]",
    stringstyle=\color{string},
    literate=
     *{0}{{{\color{numb}0}}}{1}
      {1}{{{\color{numb}1}}}{1}
      {2}{{{\color{numb}2}}}{1}
      {3}{{{\color{numb}3}}}{1}
      {4}{{{\color{numb}4}}}{1}
      {5}{{{\color{numb}5}}}{1}
      {6}{{{\color{numb}6}}}{1}
      {7}{{{\color{numb}7}}}{1}
      {8}{{{\color{numb}8}}}{1}
      {9}{{{\color{numb}9}}}{1}
      {\{}{{{\color{delim}{\{}}}}{1}
      {\}}{{{\color{delim}{\}}}}}{1}
      {[}{{{\color{delim}{[}}}}{1}
      {]}{{{\color{delim}{]}}}}{1},
}
